A Process-Theoretic Church of the Larger Hilbert Space

We show how to reconstruct a process theory of local systems starting from a global theory of reversible processes on a single global system, by using the purification principle. In such a process theory, local systems are not given, but rather `emerge' as the global system is decomposed into subsystems. Local systems thus have specific identities and their composition is naturally limited by structural constraints, a behaviour which we formalise by defining symmetric partially-monoidal categories. We reconstruct quantum theory from the global theories of unitary groups acting on projective Hilbert spaces.

==> macros.tex <==
%%%% macros.tex by Stefano Gogioso
%%%% Version 12 Apr 2017 


%% General 
	\newcommand{\emptyArg}{\,\underline{\hspace{6px}}\,} % Underscore for omitted, anonymous arguments
	\newcommand{\inlineQuote}[1]{\textquotedblleft #1\textquotedblright} % Left-right quotes surrounding #1
	\newcommand{\TODO}{\textbf{[TODO]}} % A bold TODO placeholder
	\newcommand{\citeTODO}[1]{\textbf{[#1]}} % A bold citation placeholder
	\newcommand{\goodchi}{\protect\raisebox{2pt}{$\chi$}} % A chi letter raised at line level, for those instances where alignment is an issue
	\newcommand{\goodrho}{\protect\raisebox{2pt}{$\rho$}} % A rho letter raised at line level, for those instances where alignment is an issue
	\newcommand{\goodvdots}{\protect\raisebox{7pt}{\vdots}} % A \vdots simbol raised, for use in tikz nodes where vertical alignment is a problem 
	\newcommand{\verteq}{\rotatebox{90}{$\,=$}}


%% Sets, groups and algebra
	\newcommand{\Powerset}[1]{\mathcal{P}(#1)} % Powerset of #1
	\newcommand{\naturals}{\mathbb{N}} % Set of natural numbers
	\newcommand{\integers}{\mathbb{Z}} % Set of interer numbers
	\newcommand{\circleGroup}{\mathbb{T}} % circle group
	\newcommand{\torusGroup}[1]{\circleGroup^{#1}} % #1-dimensional torus
	\newcommand{\rationals}{\mathbb{Q}} % Set of rational numbers
	\newcommand{\reals}{\mathbb{R}} % Set of real numbers
	\newcommand{\complexs}{\mathbb{C}} % Set of complex numbers
	\newcommand{\integersMod}[1]{\mathbb{Z}_{#1}} % Set/group/ring of integers mod #1
	\newcommand{\minkowskiSpace}[1]{\textbf{M}^{#1,1}} % Minkowski space with #1 space dimensios and 1 time dimension1
	\newcommand{\splitComplexs}{\mathbb{R}[\sqrt{1}]} % Ring of split complex numbers
	\newcommand{\finiteField}[1]{\mathbb{F}_{\!\!#1}} % Finite field
	\newcommand{\projectiveSpace}[2]{\operatorname{PG}(#1,#2)} % Finite projective space
	\newcommand{\modclass}[2]{#1 \; (\text{mod } #2)} % Equivalence class of integers mod #2 corresponding to representative #1
	\newcommand{\restrict}[2]{\left. #1 \right\vert_{#2}} % Restriction of function/morphism #1 to subset/subobject #2
	\newcommand{\domain}[1]{\operatorname{dom}#1} % Domain of function/morphism #1
	\newcommand{\codomain}[1]{\operatorname{codom}#1} % Domain of function/morphism #1
	\newcommand{\support}[1]{\operatorname{supp}#1} % Domain of function/morphism #1
	\newcommand{\cosupport}[1]{\operatorname{cosupp}#1} % Domain of function/morphism #1
	\newcommand{\inject}{\hookrightarrow} % Set-theoretic injection
	\newcommand{\Irreps}[1]{\operatorname{Irr}[#1]} % Set of irreps for group #1
	\newcommand{\nonstd}[1]{\,^\star #1}
	\newcommand{\starNaturals}{\nonstd{\naturals}} % Set of non-standard naturals
	\newcommand{\starIntegers}{\nonstd{\integers}} % Set of non-standard integers
	\newcommand{\starRationals}{\nonstd{\rationals}} % Set of non-standard rationals
	\newcommand{\starComplexs}{\nonstd{\complexs}} % Set of non-standard complex numbers
	\newcommand{\starReals}{\nonstd{\reals}} % Set of non-standard realsnumbers
	\newcommand{\singletonSet}{\textbf{1}}
	\newcommand{\normalSubgroup}{\trianglelefteq}
	\newcommand{\ord}[1]{{\operatorname{ord} #1}}
	\newcommand{\sgn}[2]{{\operatorname{sgn}_{#1} #2}}

%% Logic 
	\newcommand{\iffdef}{\stackrel{def}{\iff}} % If and only if (by definition)
	\newcommand{\iffdeftemp}{\stackrel{\Delta}{\iff}} % If and only if (by definition, but notation limited to section/context) 
	%\newcommand{\eqdef}{\stackrel{def}{=}} % Equal (by definition)
	\newcommand{\eqdef}{:=} % Equal (by definition)	
	\newcommand{\eqdeftemp}{\stackrel{\Delta}{=}} % Equal (by definition, but notation limited to section/context) 
	\newcommand{\imply}{\Rightarrow} % Implies
	%\newcommand{\suchthat}[2]{\left\{#1 \: \text{ s.t. } \: #2\right\}} % Set of elements #1 such that condition #2 holds 
	\newcommand{\suchthat}[2]{\left\{#1 \: \middle\vert \: #2\right\}} % Set of elements #1 such that condition #2 holds 
	\newcommand{\turnstyle}{\models} % Entails

%% Non-standard QM

	\newcommand{\stdpartSym}{\operatorname{st}}
	\newcommand{\stdpart}[1]{\stdpartSym(#1)}
	\newcommand{\indexSet}[1]{\{1,...,\dim{#1}\}}
	\newcommand{\truncate}[1]{\bar{#1}}
	\newcommand{\liftSym}[1]{\operatorname{lift}_{#1}}
	\newcommand{\lift}[2]{\liftSym{#2}[#1]}
	\newcommand{\torusAlgebra}[1]{{\SpaceH_{\,\torusGroup{#1}}}}
	\newcommand{\integersAlgebra}[1]{{\SpaceH_{\,\integers^{#1}}}}
	\newcommand{\realsAlgebra}[1]{{\SpaceH_{\,\reals^{#1}}}}
	\newcommand{\starIntegersMod}[1]{{\nonstd{\integersMod{#1}}}}
	\newcommand{\starIntegersModPow}[2]{{\nonstd{\integersMod{#1}^{#2}}}}


%% Topology, geometry and linear algebra 

	%% Inner products and traces
		\newcommand{\ket}[1]{\vert #1 \rangle} % Ket labelled #1
		\newcommand{\bra}[1]{\langle #1 \vert} % Bra labelled #1
		\newcommand{\braket}[2]{\langle #1 \vert #2 \rangle} % Inner product of bra labelled #1 with ket labelled #2
		\newcommand{\innerprod}[2]{\left( #1 , #2 \right)}
		\newcommand{\Dim}[1]{\operatorname{dim}#1} % Dimension of a space
		\newcommand{\Trace}[1]{\operatorname{Tr}\,#1} % Trace of an operator
		%\newcommand{\pTrace}[4]{\operatorname{Tr}_{#2,#3}^{#4}[#1]} % Trace of an operator
		\newcommand{\pTrace}[2]{\operatorname{Tr}_{#1}[#2]} % Trace of an operator
		\newcommand{\Norm}[2]{|| #2 ||_{#1}} % #1-norm of #2
		\newcommand{\decohSym}{\operatorname{dec}} % Decoherence map symbol
		\newcommand{\decoh}[1]{\decohSym_{#1}} % Decoherence map (for a given observable)
		\newcommand{\CPMdoubled}[1]{\textbf{double}\left[#1\right]}

	%% Kernels and images
		%\newcommand{\ker}[1]{\operatorname{ker}#1} % Kernel of a function
		\newcommand{\im}[1]{\operatorname{im}#1} % Image of a function
		\newcommand{\LinExt}[1]{\operatorname{LinExt}[#1]} % Linear extension of a function
		\newcommand{\RLinExt}[2]{#2\operatorname{-LinExt}[#1]} % R-linear extension of a function
		\newcommand{\Annihil}[1]{\operatorname{Ann}[#1]} % Annihilator subgroup of $G^\wedge$ for some subgroup $H \leq G$

	%% Sets and spans
		\newcommand{\neighborhoods}[1]{\mathfrak{N}_#1} % Set of neighborhoods of point #1
		\newcommand{\tangspace}[2]{T_{#1} \, #2} % Tangent space of point #2 in manifold #1
		\newcommand{\LinearEndoms}[1]{\operatorname{L}\left[#1\right]} % Set of linear endomorphisms of space #1
		\newcommand{\Span}[1]{\operatorname{Span}[#1]} % Span of element #1
		\newcommand{\Bounded}[1]{\operatorname{B}\left[#1\right]} % Space of bounded operators over #1
		\newcommand{\BoundedMaps}[2]{\operatorname{B}\big(#1,#2\big)} % Space of bounded operators over #1
		\newcommand{\LtwoSym}{\operatorname{L}^2} % Symbol for L2 spaces
		\newcommand{\Ltwo}[1]{\LtwoSym[#1]} % L2 space over space #1
		\newcommand{\ltwoSym}{\ell^2} % Symbol for l2 spaces
		\newcommand{\ltwo}[1]{\ltwoSym[#1]} % l2 space over space #1

	%% General purpose space names 
		\newcommand{\SpaceH}{\mathcal{H}} 
		\newcommand{\SpaceG}{\mathcal{G}}
		\newcommand{\SpaceK}{\mathcal{K}}
		\newcommand{\SpaceA}{\mathcal{A}}
		\newcommand{\SpaceB}{\mathcal{B}}
		\newcommand{\GroupG}{\mathbb{G}}
		\newcommand{\GroupH}{\mathbb{H}}
		\newcommand{\GroupK}{\mathbb{K}}


%% Category Theory 

	%% Morphisms 
		\newcommand{\isom}{\cong} % Isomorphism
		\newcommand{\iso}{\cong} % Another definition for isomorphism
		\newcommand{\epim}{\twoheadrightarrow} % Epimorphism
		\newcommand{\monom}{\rightarrowtail} % Monomorphism
		\newcommand{\id}[1]{id_{#1}} % Identity morphism of object #1
		\newcommand{\pushforward}[1]{#1_\star} % Pushforward associated with morphism #1
		\newcommand{\pullback}[1]{#1^\star} % Pullback associated with morphism #1

	%% Monoidal categories
		\newcommand{\tensor}{\otimes} % Monoidal tensor
		\newcommand{\tensorUnit}{I} % Monoidal tensor unit
		\newcommand{\cartesianTensor}{\times} % Cartesian product

	%% Homsets 
		\newcommand{\Hom}[3]{\operatorname{Hom}_{\,#1}\left[#2,#3\right]} % Set of morphisms in category #1 from object #2 to object #3
		\newcommand{\Nat}[3]{\operatorname{Nat}_{#1}[#2,#3]} % Set of natural transformations in functor category #1 from functor #2 to functor #3
		\newcommand{\Endoms}[2]{\operatorname{End}_{\,#1}\left[#2\right]} % Set of endomorphisms in category #1 for object #2
		\newcommand{\Automs}[2]{\operatorname{Aut}_{\,#1}\left[#2\right]} % Set of autoomorphisms in category #1 for object #2
		\newcommand{\Subobjs}[2]{\operatorname{Sub}_{#1}[#2]} % Set of subobjects (usually mono) in category #1 for object #2
		\newcommand{\Subsys}[2]{\operatorname{Subsys}_{#1}[#2]} % Set of subsystems (not necessarily mono) in category #1 for object #2
		\newcommand{\States}[2]{\operatorname{States}_{#1}[#2]} % Set of states in (monoidal) category #1 for object #2 
		\newcommand{\UnitaryOps}[1]{U\left[#1\right]} % Set of unitaries in a $\dagger$ category on the object #1
		\newcommand{\Isoms}[3]{\operatorname{Iso}_{\,#1}\left[#2,#3\right]} % Set of morphisms in category #1 from object #2 to object #3

	%% Canonical categories
		\newcommand{\DiffCategory}{\operatorname{Diff}} % Category of differentiable manifolds
		\newcommand{\TopCategory}{\operatorname{Top}} % Category of topological spaces
		\newcommand{\SetCategory}{\operatorname{Set}} % Category of sets
		\newcommand{\CatCategory}{\operatorname{Cat}} % Category of small categories
		\newcommand{\SitesCategory}{\operatorname{Sites}} % Category of small sites

		\newcommand{\GrpCategory}{\operatorname{Grp}} % Category of groups
		\newcommand{\fGrpCategory}{\operatorname{fGrp}} % Category of finite groups
		\newcommand{\AbCategory}{\operatorname{Ab}} % Category of abelian groups
		\newcommand{\AbGrpCategory}{\operatorname{AbGrp}} % Category of abelian groups
		\newcommand{\fAbCategory}{\operatorname{fAb}} % Category of finite abelian groups
		\newcommand{\fAbGrpCategory}{\operatorname{fAbGrp}} % Category of finite abelian groups
		\newcommand{\fMonCategory}{\operatorname{fMon}} % Category of finite monoids
		\newcommand{\fComMonCategory}{\operatorname{fCommMon}} % Category of finite commutative monoids
		\newcommand{\CMonCategory}{\operatorname{CMon}} % Category of commutative monoids
		\newcommand{\RMatCategory}[1]{#1\operatorname{-Mat}} % Category of finite sets and matrices valued in a semiring R 
		%\newcommand{\fRfreeModCategory}[1]{#1\operatorname{-Mod}_{fd}^{free}}
		\newcommand{\fRfreeModCategory}[1]{\RMatCategory{#1}} % Category of finite-dimensional free R-modules (R field, ring, semiring...)
		\newcommand{\fRModCategory}[1]{#1\operatorname{-Mod}_{fd}} % Category of finite-dimensional R-modules (R field, ring, semiring...)
		\newcommand{\RModCategory}[1]{#1\operatorname{-Mod}} % Category of R-modules (R field, ring, semiring...)
		\newcommand{\fVectCategory}[1]{#1\operatorname{-Vect}_{fd}} % Category of finite-dim R-vector spaces (R field...)
		\newcommand{\VectCategory}[1]{#1\operatorname{-Vect}} % Category of R-vector spaces (R field...)
		\newcommand{\HilbCategory}{\operatorname{Hilb}} % Category of Hilbert spaces
		\newcommand{\sHilbCategory}{\operatorname{sHilb}} % Category of separable Hilbert spaces
		\newcommand{\fHilbCategory}{\operatorname{fHilb}} % Category of finite-dimensional Hilbert spaces
		\newcommand{\fdHilbCategory}{\fHilbCategory} % Alias for the category of finite-dimensional Hilbert spaces (for retrocompatibility)
		\newcommand{\fdSubIsomsCategory}{\operatorname{fdSubIsoms}} % Category of finite-dimensional Hilbert spaces
		\newcommand{\fdCPSUCategory}{\operatorname{fdCPSU}} % Category of finite-dimensional Hilbert Spaces and Completely Positive Sub-Unital maps
		\newcommand{\RelCategory}{\operatorname{Rel}} % Category of sets and relations
		\newcommand{\PInjCategory}{\operatorname{PInj}} % Category of sets and partial injections
		\newcommand{\fRelCategory}{\operatorname{fRel}} % Category of finite sets and relations
		\newcommand{\fRelPTEP}{\operatorname{fRel}} % Process theory with environments and purification of finite sets and relations
		\newcommand{\fPInjCategory}{\operatorname{fPInj}} % Category of finite sets and partial injections
		\newcommand{\fBijCategory}{\operatorname{fBij}} % Category of finite sets and bijections
		\newcommand{\fInjCategory}{\operatorname{fInj}} % Category of finite sets and injections
		\newcommand{\fPFunCategory}{\operatorname{fPFun}} % Category of finite sets and partial functions
		\newcommand{\fPFunPTEP}{\operatorname{fPFun}} % Process theory with environments and purification of finite sets and partial functions
		\newcommand{\fSetCategory}{\operatorname{fSet}} % Category of finite sets and total functions
		\newcommand{\fFunCategory}{\fSetCategory} % Category of finite sets and total functions
		\newcommand{\fFunPTEP}{\operatorname{fFun}} % Process theory with environments and purification of finite sets and total functions
		\newcommand{\fStochCategory}{\operatorname{fStoch}} % Category of finite sets and stochastic maps
		%\newcommand{\fStochCategory}[1]{\operatorname{fStoch}_{#1}} % Category of finite sets and stochastic maps over a semiring
		\newcommand{\starHilbCategory}{^\star\!\HilbCategory} % Category of omega-truncated non-standard hilbert spaces
		\newcommand{\starHilbCategoryNearStd}{\starHilbCategory^{(std)}}
		\newcommand{\starsHilbCategory}{\nonstd{\operatorname{\sHilbCategory}}}
		\newcommand{\starsHilbCategoryNearStd}{\starsHilbCategory^{(std)}}


	%% General-purpose category names
		\newcommand{\CategoryC}{\mathcal{C}}
		\newcommand{\CategoryD}{\mathcal{D}}
		\newcommand{\CategoryM}{M}

	%% Category operators and functors
		\newcommand{\obj}[1]{\operatorname{obj} \, #1} % Set of objects of category #1
		\newcommand{\OpCategory}[1]{#1^{\operatorname{op}}} % Op-category of category #1
		\newcommand{\CategoryObjs}[1]{\operatorname{obj} \, #1} % Another notatino for the set of objects of category #1
		\newcommand{\FullSubcat}[2]{\langle #2 \rangle_{#1}} % The full subcategory of #1 generated by #2
		\newcommand{\SliceCat}[2]{#1 / #2} % Slice category obtained from category #1 over objects #2
		\newcommand{\CosliceCat}[2]{#2 \backslash #1} % Co-slice category obtained from category #1 over objects #2
		\newcommand{\Symmetries}[1]{\Automs{#1}{\emptyArg}}  % Category of symmetries of objects of category #1
		\newcommand{\LocaleCategory}[1]{\mathcal{O}(#1)} % Locale category of topological space #1
		\newcommand{\CPMCategory}[1]{\operatorname{CPM}[#1]} % Selinger's CPM category
		\newcommand{\CPCategory}[1]{\operatorname{CP}[#1]} % Bob/Chris's conjugation-independent CP construction 
		\newcommand{\CPStarCategory}[1]{\operatorname{CP}^\ast[#1]} % Chris's CP star construction
		\newcommand{\ClassicalCategory}[1]{\operatorname{K}[#1]} % Category with the same morphisms of #1, but objects pairs (object, classical structure) 
		\newcommand{\CausalSubCategory}[1]{#1_{\smallTraceSym}}
		\newcommand{\DoubledCategory}[1]{\operatorname{Double}\left[#1\right]}
		\newcommand{\KaroubiEnvelope}[1]{\operatorname{Split}\left[#1\right]} % Karoubi envelope (aka idempotent completion, or Cauchy completion) of a category
		\newcommand{\CoherentGroupsCategory}[1]{\operatorname{QG}\left[#1\right]} % Category of quantum groups in a category, and quantum groups homomorphisms
		\newcommand{\AbQuantumGroupsCategory}[1]{\operatorname{AbQG}\left[#1\right]} % Category of abelian quantum groups in a category, and quantum group homomorphisms
		\newcommand{\fQuantumGroupsCategory}[1]{\operatorname{fQG}\left[#1\right]} % Category of finite quantum groups in a category, and quantum group homomorphisms
		\newcommand{\fAbQuantumGroupsCategory}[1]{\operatorname{fAbQG}\left[#1\right]} % Category of finite abelian quantum groups in a category, and quantum group
		\newcommand{\WpAbQuantumGroupsCategory}[1]{\operatorname{wpAbQG}\left[#1\right]} % Category of bi-abelian quantum groups in a category, and quantum group homomorphisms homomorphisms
		\newcommand{\underlyingGroup}[1]{\left\llbracket#1\right\rrbracket}
		\newcommand{\dualGroupWRTMonoid}[2]{#1^{\wedge_{#2}}}
		\newcommand{\CoherentGroupRepMonad}[1]{\emptyArg \otimes #1}
		\newcommand{\RepCategory}[1]{\operatorname{Rep}\left[#1\right]}
		\newcommand{\classicalSubcategory}[1]{#1_{K}} % The classical subcategory in a probabilistic theory 



%% CQM stuff
	\newcommand{\classicalStates}[1]{K(#1)} % Classical states for a $\dagger$-qSFA
	\newcommand{\phaseGroup}[1]{P(#1)} % Phase group for a $\dagger$-qSFA
	\newcommand{\phasegate}[1]{P_{#1}}
	\newcommand{\GHZstate}[1]{GHZ_{#1}}
	\newcommand{\CPstates}[1]{\mathcal{L}[#1]}



%% Monadic dynamics

	\newcommand{\monad}{T} % General-purpose monad symbol
	\newcommand{\unit}[1]{\eta_{#1}} % Monad unit over object #1
	\newcommand{\mult}[1]{\mu_{#1}} % Monad multiplication over object #1

	\newcommand{\timeobj}{\mathbb{T}} % Time object for the monad
	\newcommand{\timeaction}{\nu} % Time-translation action of the time object over itself (for the non-uniform case)
	\newcommand{\timeunit}{\unit{}} % Initial time (unit for the time object)
	\newcommand{\timemult}{\mult{}} % Time-translation (multiplication for the time object)
	\newcommand{\timediag}{\delta} % Diagonal for the time object
	\newcommand{\timeerase}{\epsilon} % Erasure for the time object 
	\newcommand{\timeinversion}[1]{i_{#1}} % Time-inversion operation over object #1
	\newcommand{\timeinverse}{\timeinversion{}} % Time-inversion (antipode)
	\newcommand{\foliate}[1]{\operatorname{foliate}_{#1}} % Foliation map AxTB -> T(AxB)
	\newcommand{\cofoliate}[1]{\operatorname{foliate'}_{#1}} % Foliation map TAxB -> T(AxB)

	\newcommand{\freehistory}[1]{\operatorname{freehist}_{#1}} % Free history of subsystem #1
	\newcommand{\FreeHistories}[2]{\operatorname{FreeHists}_{#1}[#2]} % Set of free histories in category #1 for object #2
	\newcommand{\concretehistory}[2]{\operatorname{hist}^{#1}_{#2}} % Concrete history of sybsystem #2 under dynamic #1
	\newcommand{\ConcreteHistories}[2]{\operatorname{Hists}_{#1}[#2]} % Set of concrete histories in category #1 for object #2
	\newcommand{\ConcreteHistoriesEMCategory}[1]{\prescript{H}{}{#1}} % Eilenberg-Moore category of concrete histories

	\newcommand{\timegenerator}{\partial_t} % Generator for the time object
	\newcommand{\futurespan}[1]{\span{#1}^+} % Future span for state #1
	\newcommand{\pastspan}[1]{\span{#1}^-} % Past span for state #1
	\newcommand{\causalfuture}[2]{\operatorname{J}^+_{#1}[#2]} % Causal future for state #1
	\newcommand{\causalpast}[2]{\operatorname{J}^-_{#1}[#2]} % Causal past for state #1
	\newcommand{\dynamicGenerator}[2]{\restrict{#1}{#2}} % Restriction of propagator #1 to time state #2


%% Coarse-graining and sheaf theory

	\newcommand{\comonad}{U} % General-purpose comonad symbol
	\newcommand{\counit}[1]{\epsilon_{#1}} % Comonad counit over object #1
	\newcommand{\comult}[1]{\nu_{#1}} % Comonad comultiplication over object #1
	\newcommand{\comonadFrak}{\mathfrak{U}} % frakture comonad symbol
	\newcommand{\sheafOfEventsSym}{\mathcal{E}} % Sheaf of events symbol
	\newcommand{\sheafOfEvents}[1]{\sheafOfEventsSym[#1]} % Sheaf of events symbol
	\newcommand{\restrictionMap}[2]{\operatorname{res}^{#1}_{#2}} % Restriction map for the sheaf of events
	\newcommand{\distributionFunctorSym}[1]{\mathcal{D}_{#1}} % Functor of R-distributions (symbol)
	\newcommand{\distributionFunctor}[2]{\distributionFunctorSym{#1}[#2]} % Functor of R-distributions
	\newcommand{\presheafOfDistributionsSym}[1]{\distributionFunctorSym{#1}\sheafOfEventsSym} % presheaf of distributions (symbol)
	\newcommand{\presheafOfDistributions}[2]{\presheafOfDistributionsSym{#1}[#2]} % presheaf of distributions (functor)
	\newcommand{\supportSubpresheafSym}{\mathbb{S}} % support subpresheaf (symbol)
	\newcommand{\supportSubpresheaf}[1]{\supportSubpresheafSym[#1]} % support subpresheaf (functor)
	

%% Inline Symbols for CQM 

	%% X structure / group structure
	\newcommand{\Xcolour}{Red}
	\newcommand{\XdotSym}{\hbox{\input{symbols/XdotSym.tex}}\!} % Dot
	\newcommand{\XmultSym}{\hbox{\input{symbols/timemultSym.tex}}\!} % Multiplication
	\newcommand{\XcomultSym}{\hbox{\input{symbols/timecomultSym.tex}}\!} % Comultiplication
	\newcommand{\XunitSym}{\hbox{\input{symbols/timeunitSym.tex}}\!} % Unit
	\newcommand{\XcounitSym}{\hbox{\input{symbols/timecounitSym.tex}}\!} % Counit
	\newcommand{\antipodeSym}{\hbox{\input{symbols/antipodeSym.tex}}\!} % Antipode (group inverse)
	\newcommand{\kpoints}[1]{K_{#1}} % Classical points of a given observable
	\newcommand{\Xkpoints}{\kpoints{\XdotSym}} % Classical points for the X observable
	
	%% Z structure / point structure
	\newcommand{\Zcolour}{YellowGreen}
	\newcommand{\ZdotSym}{\hbox{\input{symbols/ZdotSym.tex}}\!} % Dot
	\newcommand{\ZmultSym}{\hbox{\input{symbols/timematchSym.tex}}\!} % Multiplication
	\newcommand{\ZcomultSym}{\hbox{\input{symbols/timediagSym.tex}}\!} % Comultiplication
	\newcommand{\ZunitSym}{\hbox{\input{symbols/timematchunitSym.tex}}\!} % Unit
	\newcommand{\ZcounitSym}{\hbox{\input{symbols/trivialcharSym.tex}}\!} % Counit
	\newcommand{\Zkpoints}{\kpoints{\ZdotSym}} % Classical points for the Z observable

	%% alternative X structure / alternative group structure (e.g. for quotients)
	\newcommand{\Xaltcolour}{Purple}
	\newcommand{\XaltdotSym}{\hbox{\input{symbols/XaltdotSym.tex}}\!}
	\newcommand{\XaltmultSym}{\hbox{\input{symbols/internaltimemultSym.tex}}\!} % Multiplication
	\newcommand{\XaltcomultSym}{\hbox{\input{symbols/internaltimecomultSym.tex}}\!} % Comultiplication
	\newcommand{\XaltunitSym}{\hbox{\input{symbols/internaltimeunitSym.tex}}\!} % Unit
	\newcommand{\XaltcounitSym}{\hbox{\input{symbols/internaltimecounitSym.tex}}\!} % Counit
	\newcommand{\Xaltkpoints}{\kpoints{\XaltdotSym}} % Classical points for the alternative X observable
	
	%% alternative Z structure / alternative point structure
	\newcommand{\Zaltcolour}{Cyan}
	\newcommand{\ZaltdotSym}{\hbox{\input{symbols/ZaltdotSym.tex}}\!}
	\newcommand{\ZaltmultSym}{\hbox{\input{symbols/internaltimematchSym.tex}}\!} % Multiplication
	\newcommand{\ZaltcomultSym}{\hbox{\input{symbols/internaltimediagSym.tex}}\!} % Comultiplication
	\newcommand{\ZaltunitSym}{\hbox{\input{symbols/internaltimematchunitSym.tex}}\!} % Unit
	\newcommand{\ZaltcounitSym}{\hbox{\input{symbols/internaltrivialcharSym.tex}}\!} % Counit
	\newcommand{\Zaltkpoints}{\kpoints{\ZaltdotSym}} % Classical points for the alternative Z observable

	%% discrete structure (aliases the black structure)
	\newcommand{\Dcolour}{black!80}
	\newcommand{\DdotSym}{\hbox{\input{symbols/DdotSym.tex}}\!} % Dot	
	\newcommand{\DcomultSym}{\hbox{\input{symbols/DcomultSym.tex}}\!} % Comultiplication	
	\newcommand{\DmultSym}{\hbox{\input{symbols/DmultSym.tex}}\!} % Multiplication
	\newcommand{\DcounitSym}{\hbox{\input{symbols/DcounitSym.tex}}\!} % Counit
	\newcommand{\DunitSym}{\hbox{\input{symbols/DunitSym.tex}}\!} % Unit

	%% X structure in B/W (black structure)

	\newcommand{\Xbwcolour}{black!80}
	\newcommand{\XbwdotSym}{\hbox{\input{symbols/DdotSym.tex}}\!\!} % Dot	
	\newcommand{\XbwcomultSym}{\!\hbox{\input{symbols/DcomultSym.tex}}\!\!} % Comultiplication	
	\newcommand{\XbwmultSym}{\!\hbox{\input{symbols/DmultSym.tex}}\!\!} % Multiplication
	\newcommand{\XbwcounitSym}{\!\hbox{\input{symbols/DcounitSym.tex}}\!\!} % Counit
	\newcommand{\XbwunitSym}{\!\hbox{\input{symbols/DunitSym.tex}}\!\!} % Unit
	\newcommand{\XbwrightcounitLawSym}{\!\hbox{\input{symbols/DrightcounitLawSym.tex}}\!\!} % Right Counit Law
	\newcommand{\XbwspecialtyLawSym}{\!\hbox{\input{symbols/DspecialtyLawSym.tex}}\!\!} % Specialty Law

	%% Z structure in B/W (white structure)
	\newcommand{\Zbwcolour}{white}
	\newcommand{\ZbwdotSym}{\hbox{\input{symbols/ZbwdotSym.tex}}\!\!} % Dot	
	\newcommand{\ZbwcomultSym}{\!\hbox{\input{symbols/ZbwcomultSym.tex}}\!\!} % Comultiplication	
	\newcommand{\ZbwmultSym}{\!\hbox{\input{symbols/ZbwmultSym.tex}}\!\!} % Multiplication	
	\newcommand{\ZbwcounitSym}{\!\hbox{\input{symbols/ZbwcounitSym.tex}}\!\!} % Counit
	\newcommand{\ZbwunitSym}{\!\hbox{\input{symbols/ZbwunitSym.tex}}\!\!} % Unit
	\newcommand{\ZbwleftDecohSym}{\hbox{\input{symbols/ZbwleftDecohSym.tex}}\!} % Left decoherence	
	\newcommand{\ZbwrightDecohSym}{\hbox{\input{symbols/ZbwrightDecohSym.tex}}\!} % Right decoherence	
	\newcommand{\ZbwunitSqNormSym}{\!\hbox{\input{symbols/ZbwunitSqNormSym.tex}}\!\!} % Squred norm of the unit

	%% Y structure in B/W (light gray structure)
	\newcommand{\Ybwcolour}{black!15}
	\newcommand{\YbwdotSym}{\hbox{\input{symbols/YbwdotSym.tex}}\!\!} % Dot	
	\newcommand{\YbwcomultSym}{\!\hbox{\input{symbols/YbwcomultSym.tex}}\!\!} % Comultiplication	
	\newcommand{\YbwmultSym}{\!\hbox{\input{symbols/YbwmultSym.tex}}\!\!} % Multiplication	
	\newcommand{\YbwcounitSym}{\!\hbox{\input{symbols/YbwcounitSym.tex}}\!\!} % Counit
	\newcommand{\YbwunitSym}{\!\hbox{\input{symbols/YbwunitSym.tex}}\!\!} % Unit

	%% W structure in B/W (dark graystructure)
	\newcommand{\Wbwcolour}{black!50}
	\newcommand{\WbwdotSym}{\hbox{\input{symbols/WbwdotSym.tex}}\!} % Dot	
	\newcommand{\WbwcomultSym}{\hbox{\input{symbols/WbwcomultSym.tex}}\!} % Comultiplication	
	\newcommand{\WbwmultSym}{\hbox{\input{symbols/WbwmultSym.tex}}\!} % Multiplication	
	\newcommand{\WbwcounitSym}{\hbox{\input{symbols/WbwcounitSym.tex}}\!} % Counit
	\newcommand{\WbwunitSym}{\hbox{\input{symbols/WbwunitSym.tex}}\!} % Unit

	%% Traces	
	\newcommand{\traceSym}{\hbox{\input{symbols/traceSym.tex}}\!} % Trace symbol
	\newcommand{\smallTraceSym}{\hbox{\input{symbols/smallTraceSym.tex}}\!} % Small trace symbol for subscripts
	\newcommand{\cotraceSym}{\hbox{\input{symbols/cotraceSym.tex}}\!} % Co-trace symbol
	\newcommand{\trace}[1]{\traceSym_{#1}} % Trace
	\newcommand{\cotrace}[1]{\cotraceSym_{#1}} % Co-trace
	\newcommand{\traceSymAlt}{\top} % Alternative trace symbol
	\newcommand{\cotraceSymAlt}{\bot} % Alternative co-trace symbol
	\newcommand{\traceAlt}[1]{\traceSymAlt_{#1}} % Alternative trace
	\newcommand{\cotraceAlt}[1]{\cotraceSymAlt_{#1}} % Alternative co-trace

	%% Unlabelled symbols for controlled dynamics (algebras), projector-valued spectra (coalgebras), etx
	\newcommand{\algebraSym}{\hbox{\input{symbols/algebraSym.tex}}\!\!}	% Gray algebra symbol (2 inputs, 1 output)
	\newcommand{\measurementSym}{\hbox{\input{symbols/measurementSym.tex}}\!\!} % The adjoint of the algebra symbol
	\newcommand{\repSym}{\hbox{\input{symbols/repSym.tex}}\!\!} % Internalised representation G -> H x H*
	\newcommand{\mapSym}{\hbox{\input{symbols/mapSym.tex}}\!\!} % The same as the measurement symbol, but with white bg.
	\newcommand{\mapconjSym}{\hbox{\input{symbols/mapconjSym.tex}}\!\!} % The conjugate of the map symbol.

%% TIKZ

	\tikzset{
	  rectangle with rounded corners north west/.initial=4pt,
	  rectangle with rounded corners south west/.initial=4pt,
	  rectangle with rounded corners north east/.initial=4pt,
	  rectangle with rounded corners south east/.initial=4pt,
	}
	\makeatletter
	\pgfdeclareshape{rectangle with rounded corners}{
	  \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
	  \inheritanchorborder[from=rectangle]
	  \inheritanchor[from=rectangle]{center}
	  \inheritanchor[from=rectangle]{north}
	  \inheritanchor[from=rectangle]{south}
	  \inheritanchor[from=rectangle]{west}
	  \inheritanchor[from=rectangle]{east}
	  \inheritanchor[from=rectangle]{north east}
	  \inheritanchor[from=rectangle]{south east}
	  \inheritanchor[from=rectangle]{north west}
	  \inheritanchor[from=rectangle]{south west}
	  \backgroundpath{% this is new
	    % store lower right in xa/ya and upper right in xb/yb
	    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
	    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
	    % construct main path
	    \pgfkeysgetvalue{/tikz/rectangle with rounded corners north west}{\pgf@rectc}
	    \pgfsetcornersarced{\pgfpoint{\pgf@rectc}{\pgf@rectc}}
	    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
	    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
	    \pgfkeysgetvalue{/tikz/rectangle with rounded corners north east}{\pgf@rectc}
	    \pgfsetcornersarced{\pgfpoint{\pgf@rectc}{\pgf@rectc}}
	    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
	    \pgfkeysgetvalue{/tikz/rectangle with rounded corners south east}{\pgf@rectc}
	    \pgfsetcornersarced{\pgfpoint{\pgf@rectc}{\pgf@rectc}}
	    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
	    \pgfkeysgetvalue{/tikz/rectangle with rounded corners south west}{\pgf@rectc}
	    \pgfsetcornersarced{\pgfpoint{\pgf@rectc}{\pgf@rectc}}
	    \pgfpathclose
	 }
	}
	\makeatother

	%% Arrowed arcs - WARNING: can cause "size" issues at compile time if arcs too small or crowded
	\tikzset{->-/.style={decoration={markings,mark=at position #1 with {\arrow{>}}},postaction={decorate}}}
	\tikzset{-<-/.style={decoration={markings,mark=at position #1 with {\arrow{<}}},postaction={decorate}}}

	\tikzstyle{every picture}=[baseline=-0.25em,scale=0.5]
	\pgfdeclarelayer{edgelayer}
	\pgfdeclarelayer{nodelayer}
	\pgfsetlayers{edgelayer,nodelayer,main}

	\tikzstyle{box} = [draw,shape=rectangle,inner sep=2pt,minimum height=6mm,minimum width=6mm,fill=white] 
	\tikzstyle{boxlarge} = [draw,shape=rectangle,inner sep=2pt,minimum height=1.5cm,minimum width=8mm,fill=white] 
	\tikzstyle{boxLarge} = [draw,shape=rectangle,inner sep=2pt,minimum height=2cm,minimum width=10mm,fill=white] 
	\tikzstyle{boxsmall} = [draw,shape=rectangle,inner sep=2pt,minimum height=3mm,minimum width=3mm,fill=white] % small in all directions. Might one day use boxnarrow for small in the largeness direction only.
	\tikzstyle{dot} = [inner sep=0mm,minimum width=3mm,minimum height=3mm,draw,shape=circle,text depth=-0.1mm]
	\tikzstyle{Zbwdot} = [dot, fill=\Zbwcolour]
	\tikzstyle{Xbwdot} = [dot, fill=\Xbwcolour]
	\tikzstyle{Ybwdot} = [dot, fill=\Ybwcolour]
	\tikzstyle{Wbwdot} = [dot, fill=\Wbwcolour]
	\tikzstyle{antipode} = [boxsmall] 

	%\tikzstyle{state} = [draw, rounded rectangle, rounded rectangle east arc=none,inner sep=2pt,minimum height=6mm,minimum width=6mm,fill=white]
	\tikzstyle{state} = [draw, rectangle with rounded corners,
	  rectangle with rounded corners north west=8pt,
	  rectangle with rounded corners south west=8pt,
	  rectangle with rounded corners north east=0pt,
	  rectangle with rounded corners south east=0pt,
	,inner sep=2pt,minimum height=6mm,minimum width=6mm,fill=white]
	\tikzstyle{statelarge} = [draw, rectangle with rounded corners,
	  rectangle with rounded corners north west=8pt,
	  rectangle with rounded corners south west=8pt,
	  rectangle with rounded corners north east=0pt,
	  rectangle with rounded corners south east=0pt,
	,inner sep=2pt,minimum height=1.5cm,minimum width=8mm,fill=white]
	\tikzstyle{stateLarge} = [draw, rectangle with rounded corners,
	  rectangle with rounded corners north west=8pt,
	  rectangle with rounded corners south west=8pt,
	  rectangle with rounded corners north east=0pt,
	  rectangle with rounded corners south east=0pt,
	,inner sep=2pt,minimum height=2cm,minimum width=8mm,fill=white]
	%\tikzstyle{effect} = [draw, rounded rectangle, rounded rectangle west arc=none,inner sep=2pt,minimum height=8mm,minimum width=6mm,fill=white]
	\tikzstyle{effect} = [draw, rectangle with rounded corners,
	  rectangle with rounded corners north west=0pt,
	  rectangle with rounded corners south west=0pt,
	  rectangle with rounded corners north east=8pt,
	  rectangle with rounded corners south east=8pt,
	,inner sep=2pt,minimum height=6mm,minimum width=6mm,fill=white]
	\tikzstyle{scalar}=[diamond,draw,inner sep=1pt,font=\small,fill=white]

	\tikzstyle{cdnode}=[fill=white]
	\tikzstyle{labelnode}=[fill=white]
	\tikzstyle{tightlabelnode}=[fill=white,inner sep = 0.1mm]
	\tikzstyle{none}=[inner sep=0pt]
	\tikzstyle{whiteline}=[-, line width=4pt, draw=white]
	%\tikzstyle{none}=[]

	\tikzstyle{trace}=[circuit ee IEC,thick,ground,scale=2.5]
	\tikzstyle{cotrace}=[circuit ee IEC,thick,ground,rotate=180,scale=2.5]
	\tikzstyle{upground}=[circuit ee IEC,thick,ground,rotate=90,scale=2.5]
	\tikzstyle{downground}=[circuit ee IEC,thick,ground,rotate=-90,scale=2.5]

	\tikzstyle{doubled} = [line width=1.8pt] % [line width=1.6pt] % [very thick]
	
	\tikzstyle{empty diagram}=[draw=gray!40!white,dashed,shape=rectangle,minimum width=1cm,minimum height=1cm]




